K\"ahler-Ricci flow on horospherical manifold

In this paper, we prove the existence of a Kahler Ricci soliton on any smooth Fano horospherical manifold by a study of the Kahler-Ricci flow. Indeed, we prove that the renormalized Kahler Ricci flow converges in the sense of Cheeger Gromov and that this limit is a Kahler-Ricci soliton.

==> macros_test.tex <==
%%%
%% Macros modifiables
%%%

% en-tête modifié

\usepackage{fancyhdr}
\fancyhead{}
\fancyfoot{}
\newcommand{\HEAD}[2]{%
\pagestyle{fancy}
\fancyhead[RO]{\scriptsize\sf\thepage}
\fancyhead[CO]{{\scriptsize\sf #1}}
\fancyhead[LE]{\scriptsize\sf\thepage}
\fancyhead[CE]{{\scriptsize\sf #2}}
%\fancyfoot[C]{\thepage}
\renewcommand{\headrulewidth}{1pt}}

% pour montrer les labels
% \usepackage[left]{showlabels}


% numérotation des équations

%\usepackage{chngcntr}
%\counterwithout{equation}{part}
%\counterwithout{equation}{section}

% numérotation des  environnements -> copier coller les macros de la section environnement selon les besoins
 
\newtheorem{prop}{Proposition}[section] 
\newtheorem{theo}[prop]{Th\'eor\`eme}
\newtheorem{lemm}[prop]{Lemme}
\newtheorem{coro}[prop]{Corollaire} 
\newtheorem{defi}[prop]{D\'efinition}

% Marges : bloc 1 si en-tête et bloc 2 si pas d'en-tête

%marge réduite au min

\usepackage[left=2.5cm,right=2.5cm,top=2cm,bottom=2cm]{geometry}

%\pagestyle{plain}
%\textwidth 15cm    
%\textheight 22.5cm 
%\oddsidemargin 0.5cm
%\evensidemargin 0.5cm
%\topmargin 0pt

%\pagestyle{plain}
%\textwidth 15cm    
%\textheight 22.5cm 
%\topmargin 30pt
% \headheight 0pt
%\headsep 0pt
% \footskip 20pt


% Police

\usepackage{palatino}
%\usepackage{bookman}
%\usepackage{lmodern}
%\usepackage{times}

%\usepackage{newcent}
%\usepackage{avant}
%\usepackage{helvet}
%\renewcommand{\familydefault}{\sfdefault}



%%%
%% Macros globales
%%%
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}     
\usepackage[francais]{babel}

\usepackage{enumerate}
\usepackage{stmaryrd}
\usepackage{amssymb} 
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{fancyhdr}


\usepackage{graphicx}
\usepackage{float}
\usepackage[all]{xy}
\usepackage{enumerate}

%%%%
%% Environnements theoremes
%%%%


%% choisir l'un des  blocs pour la numérotation 

%\newtheorem{defi}{D\'efinition}
%\newtheorem{prop}{Proposition}
%\newtheorem{theo}{Th\'eor\`eme}
%\newtheorem{conj}{Conjecture}
%\newtheorem{lemm}{Lemme}
%\newtheorem{coro}{Corollaire}



%\newtheorem{defi}{D\'efinition}[section]
%\newtheorem{prop}{Proposition}[section]
%\newtheorem{theo}{Th\'eor\`eme}[section]
%\newtheorem{conj}{Conjecture}[section]
%\newtheorem{lemm}{Lemme}[section]
%\newtheorem{coro}{Corollaire}[section]


%% raccourcis pour les environnements



\newcommand{\bdefi}{\begin{defi}}
\newcommand{\edefi}{\end{defi}}
\newcommand{\bprop}{\begin{prop}}
\newcommand{\eprop}{\end{prop}}
\newcommand{\btheo}{\begin{theo}}
\newcommand{\etheo}{\end{theo}}
\newcommand{\blemm}{\begin{lemm}}
\newcommand{\elemm}{\end{lemm}}
\newcommand{\bconj}{\begin{conj}}
\newcommand{\econj}{\end{conj}}
\newcommand{\bcoro}{\begin{coro}}
\newcommand{\ecoro}{\end{coro}}


\newcommand{\dem}{\noindent{\bf D\'emonstration. }}
\newcommand{\cqfd}{\hfill$\Box$}

\newcommand{\rem}{\noindent{\bf Remarque. }}
\newcommand{\exemp}{\medskip\noindent{\bf Exemple. }}
\newcommand{\rap}{\noindent{\bf Rappel. }}
\newcommand{\ques}{\noindent{\bf Question. }}
\newcommand{\pist}{\noindent{\bf Pistes à suivre. }}
\newcommand{\con}{\noindent{\bf Conclusion. }}

%%%%
%% Fonte \cal
%%%%


\newcommand{\A}{{\mathcal A}}
\newcommand{\R}{{\mathcal R}}
\newcommand{\I}{{\mathcal I}}
\newcommand{\T}{{\mathcal T}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\M}{{\mathcal M}}
\newcommand{\PPP}{{\mathcal P}}
\newcommand{\G}{{\mathcal G}}
\newcommand{\J}{{\mathcal J}}
\newcommand{\LLL}{{\mathcal L}}
\newcommand{\HHH}{{\mathcal H}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\K}{{\mathcal K}}
\newcommand{\OOO}{{\mathcal O}}
\newcommand{\C}{{\mathcal C}}
\newcommand{\U}{{\mathcal U}}
\newcommand{\Q}{{\mathcal Q}}
\newcommand{\F}{{\mathcal F}}
\newcommand{\V}{{\mathcal V}}
\newcommand{\W}{{ \mathcal W}}
\newcommand{\SSSS}{{\mathcal S}}
\newcommand{\N}{{\mathcal N}}


%%%%
%% Lettres mathematiques
%%%%


%% autre type d'écriture

% \usepackage{amssymb}
% \usepackage{amsmath}
% \newcommand{\maths}[1]{{\bf #1}} 


\newcommand{\maths}[1]{{\mathbb #1}}  

\newcommand{\RR}{\maths{R}}
\newcommand{\NN}{\maths{N}}
\newcommand{\CC}{\maths{C}}
\newcommand{\QQ}{\maths{Q}}
\newcommand{\BB}{\maths{B}}
\newcommand{\SSS}{\maths{S}}
\newcommand{\DD}{\maths{D}}
\newcommand{\UU}{\maths{U}}
\newcommand{\HH}{\maths{H}}
\newcommand{\MM}{\maths{M}}
\newcommand{\FF}{\maths{F}}
\newcommand{\KK}{\maths{K}}
\newcommand{\ZZ}{\maths{Z}}
\renewcommand{\AA}{\maths{A}}
\newcommand{\PP}{\maths{P}}
\newcommand{\XX}{\maths{X}}
\newcommand{\LL}{\maths{L}}
\newcommand{\TT}{\maths{T}}
\newcommand{\EE}{\maths{E}}
\newcommand{\II}{\maths{I}}

%%%%
%% Fonte gothique
%%%%


\newcommand{\aaa}{{\mathfrak a}}
\renewcommand{\ggg}{{\mathfrak g}}
\newcommand{\sss}{{\mathfrak s}}
\renewcommand{\lll}{{\mathfrak l}}
\newcommand{\ooo}{{\mathfrak o}}
\newcommand{\uuu}{{\mathfrak u}}
\newcommand{\ppp}{{\mathfrak p}}
\newcommand{\hhh}{{\mathfrak h}}
\newcommand{\fff}{{\mathfrak f}}
\newcommand{\zzz}{{\mathfrak z}}
\newcommand{\CCC}{{\mathfrak C}}
\newcommand{\nnn}{{\mathfrak n}}
\newcommand{\ttt}{{\mathfrak t}}
\newcommand{\ddd}{{\mathfrak d}}
\newcommand{\kkk}{{\mathfrak k}}
\newcommand{\bbb}{{\mathfrak b}}

\newcommand{\qqq}{{\mathfrak q}}
\newcommand{\NNN}{{\mathfrak N}}
\newcommand{\XXX}{{\mathfrak X}}
%%%%
%%  Opérateurs
%%%%

\newcommand{\id}{\operatorname{id}}
\newcommand{\Tr}{\operatorname{Tr}}
\renewcommand{\Re}{{\operatorname{Re}}}
\renewcommand{\Im}{{\operatorname{Im}}}
\newcommand{\im}{\operatorname{im}}

\newcommand{\Ric}{\operatorname{Ric}}
\newcommand{\MA}{\operatorname{MA}}
%%%%
%%  Autres
%%%%



\newcommand\refeq[1]{(\ref{#1})}

\newcommand\app[5]{
$$
\begin{array}{l|rcl}
#1 : & #2 & \longrightarrow & #3 \\
   & #4 & \longmapsto  &  #5 \end{array}
$$
}

\renewcommand{\tilde}{\widetilde}

%%%%
%%   Notes
%%%%

%faire une application :
%$$
%\begin{array}{l|rcl}
%f : & \CC & \longrightarrow & \CC \\
%   & z & \longmapsto  & f(z) \end{array}
%$$

%faire un diagramme :
%$$
%\xymatrix{
 %V \ar[rd]_{ p} \ar[r]^{t}  & V  \ar[d]^{p}\\
% & M. \\
% }\\
% $$

